State of the Art on Diffusion Models for Visual Computing

The field of visual computing is rapidly advancing due to the emergence of generative artificial intelligence (AI), which unlocks unprecedented capabilities for the generation, editing, and reconstruction of images, videos, and 3D scenes. In these domains, diffusion models are the generative AI architecture of choice. Within the last year alone, the literature on diffusion-based tools and applications has seen exponential growth and relevant papers are published across the computer graphics, computer vision, and AI communities with new works appearing daily on arXiv. This rapid growth of the field makes it difficult to keep up with all recent developments. The goal of this state-of-the-art report (STAR) is to introduce the basic mathematical concepts of diffusion models, implementation details and design choices of the popular Stable Diffusion model, as well as overview important aspects of these generative AI tools, including personalization, conditioning, inversion, among others. Moreover, we give a comprehensive overview of the rapidly growing literature on diffusion-based generation and editing, categorized by the type of generated medium, including 2D images, videos, 3D objects, locomotion, and 4D scenes. Finally, we discuss available datasets, metrics, open challenges, and social implications. This STAR provides an intuitive starting point to explore this exciting topic for researchers, artists, and practitioners alike.

==> 5_motion.tex <==
\subsection{3D Motion Generation from Motion Capture Data}\label{sec:motion} 

One of the fields that has seen a significant leap due to diffusion-based approaches is Motion Generation. 
% 
In Motion Generation, the character's shape is typically predetermined or restricted, and its motion is controlled by a low-dimensional parametric human body model. 
% 
Most commonly, the motion parameters of this model describe rotation angles or positions of skeleton joints (with another set of parameters controlling shape through mechanisms like linear-blend-skinning) \cite{SMPL:2015,SMPL-X:2019}. 
% 
Perhaps the reason diffusion approaches have brought a leap for this field is the structure of the domain: When considering the text-to-motion task, many ambiguities arise regarding the relation between the input and output; 
% 
A motion can be described in many ways (e.g., ``standing up from a crouch with hands raised above head'' vs. ``lifting weights''), and many motions typically satisfy the same description (e.g., ``running'' could be fast or slow, light or frantic, with specific striding styles and other variations difficult to capture with text). 
% 
Hence, a distribution-to-distribution generative approach is warranted, which aligns nicely with the diffusion framework. 
% 
With respect to data, there is a high interest in capturing 3D human motions, as those can be used in a plethora of computer graphics applications (such as virtual character animation, motion transfer, motion prediction and movie production) and they are necessary to address different computer vision problems (e.g., monocular human pose estimation). 
% 
Consequently, the community has 
% amassed 
produced 
% many 
different datasets of human motion capture such as the ones united in AMASS \cite{mahmood2019amass}. 
% 
Even though they are still far from properly spanning the entire human motion manifold, they contrast with several other research fields that experience a more severe lack of 3D and 4D data ({cf.} Sec.~\ref{sec:4dnerf}). 
% 
% Hence, this is in strong contrast to many other research fields that experience a lack of 3D or 4D data ( {cf.} Sec.~\ref{sec:4dnerf}). 
% 
% Amit.Bermano: I guess this is true for 4D, but I'm not sure this is the case for 3D. At the end of the day there isn't that much data in motion and it doesn't span the human manifold properly. I would drop the last sentence I think altogether. 
% 




% human motions can be captured 


    % 
Indeed, even before recent advancements, motion generation was mostly dominated by the VAE architecture \cite{petrovich2021action,zhang2023generating,petrovich2022temos,tevet2022motionclip,ahuja2019language2pose,holden2016deep}, with little work employing the more popular GANs method \cite{raab2023modi,barsoum2018hp,hernandez2019human,aberman2020unpaired}. 
% 
This is again aligned with the premise that the single-to-single matching setting of GANs is less suitable for this domain. 
% 
In contrast, diffusion models are well-suited for this task as they model complicated data distributions and provide desired variations for the motion generation task.
%, which was demonstrated experimentally. 
% 

% 31.08.2022: MotionDiffuse 
% 01.09.2022: FLAME 
% 29.09.2022: MDM 
% 19.11.2022: EDGE 
% 08.12.2022: MoFusion 
% 09.12.2022: MoFusion of Ma  {et al.} 

% 
The first pioneers to introduce diffusion to motion generation concurrently were MotionDiffuse \cite{zhang2022motiondiffuse}, FLAME \cite{kim2023flame}, MDM \cite{Tevet2023}, EDGE \cite{tseng2023edge}, and two papers calling their method MoFusion \cite{dabral2022mofusion,Ma2022}. 
%, and MoFusion of Ma  {et al.}~\cite{Ma2022}
% \cite{zhang2022motiondiffuse,kim2023flame,Tevet2023,dabral2022mofusion}. 
% 
Unlike the convolutional U-Net architecture typically used for diffusion-based generation, these works offer a transformer-based framework, as it better encodes the symmetries of the skeleton-structured input domain (vs.~the 2D symmetry of images for example). 
% 
In addition, the methods also offer editing capabilities that are similar to those seen in classical domains such as 2D images. 
% 
These include inpainting (performed temporally) as in-betweening or motion bootstrapping, or spatially as motion completion. 
% FLAME, MDM, EDGE, MoFusion and Ma  {et al.} offer a transformer-based framework, whereas ... 
% 
%MDM \cite{Tevet2023} is a classifier-free diffusion-based generative model with a transformer for 3D human motion synthesis. 
% 
In MDM \cite{Tevet2023}, samples are predicted directly instead of predicting noise in each diffusion step, which simplifies the usage of established geometric losses (e.g., foot contact losses),  commonly used in inverse problems and generative tasks involving 3D human motions. 
% 
In contrast to them, MoFusion~\cite{dabral2022mofusion} is designed for the synthesis of 3D human motions both from textual or raw audio inputs (music samples). 
% 
The paper shows how common soft constraints on 3D human poses---such as the temporal variance of bone lengths and right-left skeleton asymmetries---can be integrated into the proposed approach for better consistency and generative quality. 
% 
% MoFusion \cite{dabral2022mofusion} allows for various conditions, including music. 
% They also incorporate geometric losses through soft weighting. 

% 
Since then, many works improved upon them and addressed further aspects of motion generation less common in classical diffusion domains, including scenarios with human-object interactions \cite{kulkarni2023nifty}, 
incorporation of spatial constraints (e.g., pre-defined motion trajectories and obstacles) \cite{Karunratanakul2023}, 
gesture generation 
%as an important category of human motions 
\cite{yang2023diffusestylegesture, Yin2023, Zhang2023DiffMotion}, 
conditioning on 
% a wide variety of signals 
sparse tracking signals \cite{Du2023}, 
physics-based corrections during the diffusion process to mitigate physically implausible artefacts 
% make the generated motions plausible 
\cite{Yuan2023}, 
motion generation with interactions for multiple humans \cite{Liang2023}, 
long-term and arbitrary long motion synthesis \cite{zhang2023tedi, Shafir2023} as well as 
synthesis from a single exemplary sequence \cite{Raab2023arXiv}. 
% 
Some methods focus exclusively on dance motion generation, such as EDGE \cite{tseng2023edge} or 
% Listen, Denoise, Action! 
Alexanderson {et al.}~\cite{Alexanderson2023}, 
% pairs (text, static pseudo poses) extracted from image-text datasets \cite{azadi2023make} 
and some leverage 2D image-text datasets instead of 3D datasets only for improved characteristics of the synthesised motions \cite{azadi2023make} or refine the denoising diffusion with retrieval of motions from a database \cite{Zhang_2023_ICCV}. 
% 

% 
%The existing approaches achieve all that through technical innovations tailored to the specific scenarios. 
% 
% All these methods 
These diffusion-based approaches collectively demonstrate motion quality that was not seen before in the field, with generalizability, editability and natural language control that are revolutionary compared to the state-of-the-art beforehand. 
% 


% Classification: Unconditional Motion Generation; Long-term motion synthesis; Text- and Music-to-Dance; Gesture and Multi-Modal Generation (includes multiple humans and interactions between them); Motion generation with Spatial Constraints. 
% 


% 
\paragraph*{Text- and Music-to-Dance Generation.} 
% 
% Consider and discuss music-to-dance and co-speech gesticulation, and gestures together? 
% 
% 
Some methods generate motions from different signals including audio, or are explicitly designed for motion and dance synthesis from audio signals. 
% 
EDGE \cite{tseng2023edge} is a transformer-based diffusion model paired with a pre-trained music feature extractor Jukebox \cite{Dhariwal2020}---acting as cross-attention context---for realistic dance motion generation. 
% 
EDGE offers versatile editing functionality 
%such as motion/dance in-betweening and temporal and joint-wise motion generation constraints; 
and arbitrary long sequences. 
%can also be generated through editing. 
% 
This is possible by replacing the known regions with forward-diffused samples of the provided constraint (through masking), which is an increasingly popular technique enabling editability at test time without the need for model retraining. 
% 
% motion/dance in-betweening and joint-wise conditioning 
% but there is no explicit physical modeling 
% arbitrary long sequences! 
% 
% A NEW METRIC FOR PHYSICAL PLAUSIBILITY 
% also for the metrics section 
% beat alignment 
% realistic and physiall plausilbe dance motions based on input music 
% 
Listen, Denoise, Action!~\cite{Alexanderson2023} is a method based on a stack of Conformers for dance motion generation from audio signals. 
% 
It takes acoustic feature vectors and an optional style vector as inputs. 
% 
% Alexanderson  {et al.}~\cite{Alexanderson2023}, 
% co-speech articulation 
% 
The method enables control over motion style with classifier-free guidance and dance style interpolation thanks to the product-of-experts ensembles of diffusion models (guided interpolation of different probability distributions). 
% 
See Fig.~\ref{fig:Alexanderson_etal_2023} for exemplary results by Alexanderson {et al.}'s method \cite{Alexanderson2023}. 
% 
% 
Next, MoFusion \cite{dabral2022mofusion} conditions human dance generation on Mel spectrograms. 
% 
The advantage of the latter is that the context embedding layer of the MoFusion architecture learns a suitable injection of the audio signal to the feature space of a U-Net, in contrast to MFCC features that offer less flexibility. 
% 
% MoFusion uses Mel spectrograms for music conditioning, which allows the context embedding layer to learn the projection to the feature space of U-Net; it also allows the method to be trained with other audio signals such as speech. 

% given audio 
% DiffWave 
% control over motion style with classifier-free guidance 

% gesture and dance generation 
% product-of-expert ensembles of diffusion models for style interpolation 

% 
\paragraph*{Motion Generation with Spatial Constraints.} 
% conditioned on trajectories; physics-based 
% 
Integration of spatial constraints into 3D human motion generation with diffusion models is another active research direction. 
% 
% Constraints other than physics-based 
% GMD Guided Motion Diffusion for Controllable Human Motion Synthesis, Karunratanakul et al. 
GMD \cite{Karunratanakul2023}, for example, offers two elaborate mechanisms to allow spatial conditioning including trajectory, keypoints and obstacle avoidance objectives. 
%  
% They allow trajectory, keypoint locations, and obstacle avoidance. 
% 
NIFTY's architecture \cite{kulkarni2023nifty} includes an object interaction field that guides the motion generator to enable the support of human-object interactions. 
% nifty - adds a condition on MDM to interact with objects through an interaction field 
% Avatars Grow Legs Du et al. 
AGRoL~\cite{Du2023} is an MLP-based architecture with a conditional diffusion model for full-body motion synthesis accepting a sparse upper-body tracking signal. 
% 
The method supports real-time inference rates, which places them among only a few techniques well-suitable for AR and VR applications. 
% 
% two virtual characters  
InterGen \cite{Liang2023} is a model generating interactive human motions. 
% 
The paper considers the case of two virtual characters constraining each other's movements. 
% 
InterGen's objective is reflected in its architecture: It contains cooperative denoisers that share weights and a mutual attention mechanism, which improves the motion generation quality. 
% 
Additional interaction regularizers (losses) with a damping schedule allow modeling of complex spatial relations between the generated motions. Similarly, Shafir et al.~\cite{Shafir2023} train a slim communication layer to synchronize two pre-trained motion models using only a few training examples. In a similar vein, BUDDI~\cite{mueller2023buddi} focuses on generating the pose, shape, and global translation of two people in close proximity. In particular, this approach learns the diffusion model directly in the SMPL parameter space, instead of the 3D joint space. The diffusion model is learned from pseudo-ground truth obtained from image with contact annotations, and the resulting model is used for reconstructing two people in close contact from a single image. 
% 


% Physics-based Constraints 
% contact consistency loss, intuitive physics 
% 
Several approaches integrate constraints in human motion capture that were recently conjointly dubbed as ``intuitive physics'' \cite{McCloskey1983, Tripathi2023}. 
% 
Thus, EDGE follows a set of simplified rules approximating diverse physical laws: Along the axes of the ground plane, center of mass (CoM) of the human can only be accelerated by static contacts between at least one foot and the ground. 
% 
Along the vertical axis, any positive CoM acceleration is due to static foot contacts. 
% 
EDGE also proposes to maintain the bone lengths of the virtual character in each generation motion sequence. 
% , which is a term similar to the one used in MoFusion \cite{dabral2022mofusion}. 
% 
Similarly, MoFusion \cite{dabral2022mofusion} explicitly penalises deviations in the bone lengths across the generated motion sequences. 
% 


% 
% Along the axes of the ground plane: Center of mass acceleration is due to static contact between the feet and the ground 
% Hence, at least one foot must be stationary on the ground for the COM accelerating. 
% Along the vertical axis: 
% 
% maintain bone length (the same as MoFusion), they must be fixed 
% aspects of physical plausibility in EDGE and TEvet et al.: 
% joint positions (Eq. (3)), velocities (Eq. (4)), and foot velocities via our Contact Consistency Loss 
% 
% metric: beat alignment score 


% physics-guided motion diffusion 
% injecting physical laws into the diffusion process 
% 
PhysDiff \cite{Yuan2023} goes a different way beyond geometric priors, namely physics-guided motion diffusion: It adds a physics-based motion projection step into the diffusion process of existing methods that mitigates such artefacts as floating in the air, foot-floor penetration and foot sliding. 
% 
The projection step of PhysDiff is a human motion imitation policy controlling a virtual character in a physical simulator and enforcing the physical constraints. 
% 
% PhysDiff \cite{Yuan2023} goes beyond geometric priors and adds a physics-based motion projection step for physics-guided motion diffusion. 
% PhysDiff's motion projection includes an imitation policy in combination with a physics simulator. 
% denoiser can be any mnotion denoising network 
% 



% 
\paragraph*{Long-term Motion Synthesis.} 
% 
The TEdi approach \cite{zhang2023tedi} entangles the time-axis of diffusion and temporal motion axis: In each diffusion step of their stationary motion buffer (a.k.a.~pre-defined motion generation window), 
% diffusion time-axis 
they remove a clean frame at the beginning of the buffer and append a new noise vector to its end. 
%  TEDi~\cite{zhang2023tedi} entangles the time-axis of diffusion and the temporal-axis of motion to generate long-term sequences, instead of fixed-length sequences. 
% 
As a result, the method can generate arbitrary long motion sequences in an autoregressive manner. 
% 
A different approach is pursued by DoubleTake, \cite{Shafir2023} that extends MDM for long-term motion synthesis without additional training. 
% 
% DiffusionBlending 
Their sequential composition approach concatenates short motion sequences with a diffusion blending step (performed in a zero-shot manner): In the first ``take'', their method generates motion batches and the second ``take'' refines the transitions between individual motions. 
% the prior is trained from short clips only 
Their motion prior is trained from short 3D motion clips only, and the method allows individual control of each motion interval. 
% 


% 
In addition to the methods discussed above, several other techniques include components supporting the generation of long sequences. 
% 
% Last but not least, 
Thus, MoFusion \cite{dabral2022mofusion} can generate long motion using seed conditioning in a sliding window fashion. 
% 
% the seed frames are not denoised 
% 
The provided seed motion frames are first corrupted by noise, while the remaining ones that need to be generated are initialised with random noise. 
% 
At each denoising step, the seed frames are masked out, which eventually leads to generated motions complementing the seed motions. 
% 
A similar policy is also applicable to MotionDiffuse \cite{zhang2022motiondiffuse}, MDM \cite{Tevet2023} and EDGE \cite{tseng2023edge}. 
% 
Similarly to DoubleTake \cite{Shafir2023}, EDGE \cite{tseng2023edge} synthesises multiple motion sequences and edits them to concatenate them and enforce temporal consistency. 
% 
Note that generally, this approach is simple but is inherently limited in that it can capture local dependencies only (but not choreographies with extended contexts)\cite{tseng2023edge}. 
% 
In Alexanderson {et al.}~\cite{Alexanderson2023}, translation-invariant policy to encode positional information enables better generalisation to long sequences. 
% 



\paragraph*{Gesture and Multi-Modal Motion Generation.} 
% includes multiple humans and interactions between them 

% 
Gesture generation approaches use speech as a condition along with text for style; the attention mechanism is leveraged to synchronise the gestures to the speech. 
% Both are attended into the generative process like a condition, but here the attention mechanism is leveraged to synchronise the gestures to the speech. 
% 
% 
The approach of Deichler {et al.}~\cite{Deichler2023arXiv} proposes a contrastive speech and motion pre-training module that learns joint embedding of speech and gesture; it learns a semantic coupling between these modalities. 
% 
% DiffuseStyleGesture: Stylized Audio-Driven Co-Speech Gesture Generation with Diffusion Models 
DiffuseStyleGesture \cite{yang2023diffusestylegesture} is an audio-driven co-gesture generation approach that synthesises gestures matching the music rhythm and text descriptions based on cross-local and self-attention mechanisms. 
% 
It uses classifier-free guidance to manipulate the initial gestures and interpolate or extrapolate them. 
% 
EMoG \cite{Yin2023} decomposes the generation problem into two steps, i.e., joint correlation and temporal dynamics, and shows that explicitly predicting joint correlation improves generation quality. 
% 
% 
% emog - they decompose the generation problem into two steps - joint correlation and temporal dynamics, and show that explicitly predicting joint correlation improves generation quality. So they play with conditioning mechanisms to get better "integrate emotion into the gesture". 
% DiffMotion: Speech-Driven Gesture Synthesis Using Denoising Diffusion Model 
DiffMotion \cite{Zhang2023DiffMotion} is a two-stage framework for speech-driven gesture synthesis. 
% 
Its auto-regressive temporal encoder (LSTM-based) conditions the diffusion module on temporal dynamics extracted from the preceding human poses (gestures) and acoustic speech features. 
% 


% \paragraph*{} 
% 

% 
% The existing approaches achieve all that through technical innovations tailored to the specific scenarios. 
% 
% MDM \cite{Tevet2023} is a classifier-free diffusion-based generative model with a transformer for 3D human motion synthesis. 
% 
% Instead of predicting noise in each diffusion step, it predicts samples directly, which simplifies the usage of geometric losses ( {e.g.,} foot contact losses) that are widely used in inverse problems and generative tasks involving 3D human motions. 
% 
% TEDi~\cite{zhang2023tedi} entangles the time-axis of diffusion and the temporal-axis of motion to generate long-term sequences, instead of fixed-length sequences. 
%
% Alexanderson  {et al.}~\cite{Alexanderson2023} investigate music-to-motion generation (Fig.~\ref{fig:Alexanderson_etal_2023}), whereas 
% Zhang  {et al.}~\cite{Zhang2023DiffMotion} focus on speech-driven gesture synthesis. 
% 
% In contrast to them, MoFusion~\cite{dabral2022mofusion} is designed for the synthesis of 3D human motions both from textual or raw audio inputs (music samples). 
% 
% MoFusion uses Mel spectrograms for music conditioning, which allows the context embedding layer to learn the projection to the feature space of U-Net; it also allows the method to be trained with other audio signals such as speech. 
% 
% Dabral  {et al.}~\cite{dabral2022mofusion} show how common soft constraints on 3D human poses---such as the temporal variance of bone lengths and right-left skeleton asymmetries---can be integrated into the proposed approach. 
% 
% PhysDiff \cite{Yuan2023} goes beyond geometric priors and adds a physics-based motion projection step for physics-guided motion diffusion. 
% 
% PhysDiff's motion projection includes an imitation policy in combination with a physics simulator. 
% 
% NIFTY \cite{kulkarni2023nifty} includes an object interaction field that guides the motion generator to enable the support of human-object interactions. 
% 

% estimation of noise in each step versus estimation of the target signal 
% 




%These works 
%[were alike this ways handled humans, offered the same architecture? had the same principles? ], 
%but [were different this way. no 1 had a special feature, no 2 and 3 another. no 4 has yet a different insight. mdm adds geometric losses through x0. ] 
% 
% All these methods demonstrated motion quality that was not seen before in the field, with generalizability and natural language control that was revolutionary to the capabilities at the time. editing - similar to images. 
% 
% key difference - physics (geometric losses). Mdm offers one way, mofusion another. 
% -> other music 
% -> edge 
% -> other tricks in diffusion process (physdiff) -> prior

% sinmdm 
% Single Motion Diffusion \cite{Raab2023arXiv}: Learning from a single input motion. 
% 
% the archutecture is a shallow network with local attention layers that narrrow the receptive field and encourage motion diversity 
% 


% Possible references:
% MoFusion~\cite{dabral2022mofusion}, 
% MotionDiffuse~\cite{zhang2022motiondiffuse}.
% Gesture generation~\cite{yang2023diffusestylegesture}.
% MDM \cite{Tevet2023} 
% EMoG \cite{Yin2023} 
% Listen, Denoise, Action! \cite{Alexanderson2023} 
% GMD Guided Motion Diffusion for Controllable Human Motion Synthesis, Karunratanakul et al. \cite{Karunratanakul2023} 
% Avatars Grow Legs Du et al. \cite{Du2023}
% InterGen \cite{Liang2023} 
% Human Motion Diffusion as a Generative Prior \cite{Shafir2023} 
% Single Motion Diffusion \cite{raab2023single} 
% DiffMotion: Speech-Driven Gesture Synthesis Using Denoising Diffusion Model \cite{Zhang2023DiffMotion} 
% Pretrained Diffusion Models for Unified Human Motion Synthesis \cite{Ma2022} 
% DiffuPose: Monocular 3D Human Pose Estimation via Denoising Diffusion Probabilistic Model \cite{choi2022diffupose}? 
% PhysDiff \cite{Yuan2023} 
% Make-an-animation: Large-scale text-conditional 3d human motion generation \cite{azadi2023make}
% TEDi: Temporally-Entangled Diffusion for Long-Term Motion Synthesis \cite{zhang2023tedi}
%edge \cite{tseng2023edge}
% FLAME: Free-form Language-based Motion Synthesis \& Editing \cite{kim2023flame} 


% MoFusion - allows for various conditions, including music. They try to incorporate geometric losses through soft weighting. 
% motionDiffuse, flame - classic.
% flame and mdm offer a transformer based framework.
% Gesture generation - use speech as condition along with text for style. both are attended into the generative process like a condition, but here the attention mechanism is leveraged to sync the gestures to the speech. 
% nifty - adds a condition on MDM to interact with objects through an interaction field
% emog - they decompose the generation problem into two steps - joint correlation and temporal dynamics, and show that explicitly predicting joint correlation improves generation quality. So they play with conditioning mechanisms to get better "integrate emotion into the gesture". 
% Listen, Denoise, Action! \cite{Alexanderson2023} - investigate music-to-motion generation. not much to add. They show dance and gestures.
% gmd - two elaborate mechanisms to allow spatial conditioning. they allow trajectory, keypoint locations, and obstacle avoidance.
%diffmotion - 
%ma2022 - 
%magicpony -
%make-an-animation - 
%TEDi~\cite{zhang2023tedi} entangles the time-axis of diffusion and the temporal-axis of motion to generate long-term sequences, instead of fixed-length sequences.
%Avatars Grow Legs - 
%InterGen - 



%Recognizing that DDPMs can be efficiently used for 3D human motion synthesis from various signals led to several concurrent works \cite{Tevet2023, zhang2023tedi, dabral2022mofusion, zhang2022motiondiffuse, Alexanderson2023, Zhang2023DiffMotion, Yuan2023}. 
% 
%All these methods using DDPMs demonstrate improved generalizability and motion realism compared to previous techniques that do not rely on DDPMs. 
% 



% 
\paragraph*{Summary.} 
% 
To summarise, diffusion models recently became the main factor in significant improvements in 3D human motion generation demonstrated by recent techniques. 
% 
The proposed (predominantly transformer-based) techniques allow conditioning motion generation on a wide range of signals such as text, music or speech. 
% 
In addition, the iterative nature of the diffusion process is leveraged in several ways by the reported methods to incorporate more elaborate signals such as temporal consistency or physical plausibility. 
% 
We have seen methods accounting for spatial and physics-based constraints as well as two-person interactions. 
% 
In long-term motion synthesis, capturing global and long-term context remains an open challenge, as most methods generate short motion sequences that are then stitched into longer ones. 
% 
We believe that the demonstrated characteristics suggest 
that motion planning (e.g., for virtual characters in computer games) and crowd simulation (i.e., motion generation with significantly more than two virtual characters) could benefit from diffusion models. 
% 
We also anticipate more work in future on the multi-modal generation of human gestures, motions, speech and appearance with diffusion models. 
% 



\begin{figure}[t] 
	\begin{center} 
        \includegraphics[width=\linewidth] {figures/Alexanderson_etal_2023.png} 
	\end{center} 
	\caption{\textbf{Motion Generation.} Dances synthesised from audios by the approach of Alexanderson et al.~\cite{Alexanderson2023} for Locking (top row) and Krumping (bottom row) dance styles. Image reproduced from \cite{Alexanderson2023}.} 
	\label{fig:Alexanderson_etal_2023} 
\end{figure} 

==> bios.tex <==
\section{\textbf{Contributor Biographies}}

\noindent
\textbf{Ayush Tewari} is a recent Ph.D. graduate in the `Visual Computing and Artificial Intelligence' department at the Max Planck Institute for Informatics in Saarbr\"ucken, Germany. His research interests are in computer vision, computer graphics, and machine learning, with a focus on self-supervised 3D reconstruction and rendering. 

\noindent
\textbf{Justus Thies} is an independent research group leader at the Max Planck Institute for Intelligent Systems in Tübingen, Germany (MPI-IS). His group `Neural Capture \& Synthesis' works at the intersection of computer graphics, computer vision, and machine learning, focusing on digital humans in motion. Specifically, he is interested in capturing and (re-)synthesizing the real world using commodity hardware. This includes marker-less motion capturing and 3D reconstruction of facial performances, human bodies, and general non-rigid objects, as well as AI-based synthesis techniques that allow for photo-realistic image and video synthesis.

\noindent 
\textbf{Ben Mildenhall} is a research scientist at Google, where he works on problems at the intersection of graphics and computer vision, specializing in view synthesis and inverse rendering. He received his PhD in Computer Science from UC Berkeley in 2015, where he was advised by Ren Ng and supported by a Hertz Foundation Fellowship, and he received his BS from Stanford University in 2015. He received the David J. Sakrison Memorial Prize in 2021, the Tong Leong Lim Pre-Doctoral Prize in 2017, and a Best Paper Honorable Mention at ECCV 2020 and ICCV 2021.

\noindent
\textbf{Pratul Srinivasan} is a research scientist at Google Research, where he works on problems at the intersection of computer vision, computer graphics, and machine learning. His recent work focuses on view synthesis and inverse rendering. Pratul received his PhD from the EECS Department at UC Berkeley in December 2020, where he was advised by Ren Ng and Ravi Ramamoorthi and supported by an NSF Graduate Fellowship.  He received the David J. Sakrison Memorial Prize from UC Berkeley in 2021, the ECCV Best Paper Honorable Mention Award in 2020, and the ICCV Best Paper Honorable Mention Award in 2021. 


\noindent
\textbf{Edith Tretschk} is a fourth-year Ph.D.~student in the `Visual Computing and Artificial Intelligence' department at the Max Planck Institute for Informatics in Saarbr\"ucken, Germany. She received her B.Sc.~in Computer Science from Saarland University. Her research interests are at the intersection of computer vision, computer graphics, and machine learning. Her focus is on 3D reconstruction problems, especially general non-rigid objects from image or video inputs.

\noindent
\textbf{Wang Yifan} is a postdoc at Stanford University. Her area of research lies in applying machine learning techniques, especially deep learning, to challenging image and geometry processing problems. She received her PhD from ETH Zurich, advised by Professor Olga Sorking-Hornung. She was awarded the Apple AI/ML fellowship in 2020.

\noindent
\textbf{Christoph Lassner} is  a  Research  Scientist  at  Facebook  Reality Labs Research  (FRLR)  in  Sausalito. He works towards better means of interaction between humans and machines---this involves in particular creating physically accurate models of humans and our world, and being able to reproduce them faithfully and swiftly in the virtual world. Achieving this requires technologies ranging from computer vision over computer graphics to machine learning and simulation and, naturally, neural rendering. Before joining Facebook, Christoph worked at Bodylabs and Amazon on 3D and 2D body pose and shape estimation technology. He received his PhD from the University of T\"ubingen, where he was a PhD student at the Bernstein Center for Computational Neuroscience and the Max-Planck Institute for Intelligent Systems.

\noindent
\textbf{Vincent Sitzmann} is an incoming Assistant Professor at MIT CSAIL. Currently, he's a postdoc with Joshua Tenenbaum, William Freeman, and Fredo Durand. Previously, he finished his PhD at Stanford University. His primary research interests lie in the self-supervised learning of neural representations of 3D scenes, and their applications in computer graphics, computer vision, and robotics.

\noindent
\textbf{Ricardo Martin-Brualla} is a researcher at Google Seattle, where he currently works at the intersection of computer vision, computer graphics, and machine learning, developing new capture and rendering techniques of humans. He completed his PhD in Computer Science from the University of Washington in 2016, where he was advised by Steve Seitz, his and BSc and BEng degrees in Mathematics and Computer Engineering from the Universitat Polit\`ecnica de Catalunya in 2010 and 2011. He received the La Caixa Fellowship in 2010, and the Best Paper Honorable Mention at ICCV 2021.

\noindent
\textbf{Stephen Lombardi} is a Research Scientist at Facebook Reality Labs Research (FRLR) in Pittsburgh. He received his Bachelors in Computer Science from The College of New Jersey in 2009, and his Ph.D. in Computer Science, advised by Ko Nishino, from Drexel University in 2016. His doctoral work aimed to infer physical properties, like the reflectance of objects and the illumination of scenes, from small sets of photographs. At FRLR, he developed realistic, driveable models of human faces by combining deep generative modeling techniques with 3D morphable models. His current research interests are the unsupervised learning of volumetric representations of objects, scenes, and people.

\noindent
\textbf{Tomas Simon} is a Research Scientist at Facebook Reality Labs Research (FRLR) in Pittsburgh. He received his Ph.D. in 2017 from Carnegie Mellon University, advised by Yaser Sheikh and Iain Matthews. He holds a B.S. in Telecommunications from Universidad Politecnica de Valencia and an M.S. in Robotics from Carnegie Mellon University, which he obtained while working at the Human Sensing Lab advised by Fernando De la Torre. His research interests lie mainly in using computer vision and machine learning to model faces and bodies.


\noindent
\textbf{Christian Theobalt} is a Professor of Computer Science and the Director of the Visual Computing and Artificial Intelligence Department at the Max Planck Institute for Informatics, Saarbruecken, Germany. He is also a professor at Saarland University. His research lies at the Intersection of Computer Graphics, Computer Vision and Machine Learning. For instance, he works on virtual humans, 3D and 4D scene reconstruction, neural rendering and neural scene representations, marker-less motion and performance capture, machine learning for graphics and vision, and new sensors for 3D acquisition. Christian received several awards, for instance the Otto Hahn Medal of the Max-Planck Society (2007), the EUROGRAPHICS Young Researcher Award (2009), the German Pattern Recognition Award (2012), the EURIGRAPHICS Outstanding Technical Contributions Award (2020), an ERC Starting Grant (2013) and an ERC Consolidator Grant (2017). He is a co-founder of theCaptury (www.thecaptury.com). 


\noindent
\textbf{Matthias Nie{\ss}ner} is a Professor at the Technical University of Munich where he leads the Visual Computing Lab. Before, he was a Visiting Assistant Professor at Stanford University. Matthias’s research lies at the intersection of computer vision, graphics, and machine learning, where he is particularly interested in cutting-edge techniques for 3D reconstruction, semantic 3D scene understanding, video editing, and AI-driven video synthesis. In total, he has published over 100 academic publications, including 25 papers at the prestigious ACM Transactions on Graphics (SIGGRAPH / SIGGRAPH Asia) journal and 49 works at the leading vision conferences (CVPR, ECCV, ICCV); several of these works won best paper awards, including at SIGCHI’14, HPG’15, SPG’18, and the SIGGRAPH’16 Emerging Technologies Award for the best Live Demo.




\noindent
\textbf{Jonathan T. Barron} is a senior staff research scientist at Google, where he works on computer vision and machine learning. He received a PhD in Computer Science from the University of California, Berkeley in 2013, where he was advised by Jitendra Malik, and he received a Honours BSc in Computer Science from the University of Toronto in 2007. He received a National Science Foundation Graduate Research Fellowship in 2009, the C.V. Ramamoorthy Distinguished Research Award in 2013, the PAMI Young Researcher Award in 2020, and the Best Paper Honorable Mention at ECCV 2016, ECCV 2020, and ICCV 2021. His works have been selected as a focus paper for TPAMI (2016) and featured as a research highlight by the Communications of the ACM (2022).

\noindent
\textbf{Gordon Wetzstein} is an Associate Professor of Electrical Engineering and, by courtesy, of Computer Science at Stanford University. He is the leader of the Stanford Computational Imaging Lab and a faculty co-director of the Stanford Center for Image Systems Engineering. At the intersection of computer graphics and vision, computational optics, and applied vision science, his research has a wide range of applications in next-generation imaging, display, wearable computing, and microscopy systems. He is the recipient of an NSF CAREER Award, an Alfred P. Sloan Fellowship, an ACM SIGGRAPH Significant New Researcher Award, a Presidential Early Career Award for Scientists and Engineers (PECASE), an SPIE Early Career Achievement Award, a Terman Fellowship, an Okawa Research Grant, the Electronic Imaging Scientist of the Year 2017 Award, an Alain Fournier Ph.D. Dissertation Award, and a Laval Virtual Award as well as Best Paper and Demo Awards at ICCP 2011, 2014, and 2016 and at ICIP 2016. 

\noindent
\textbf{Michael Zollhoefer} is a Research Scientist at Facebook Reality Labs Research (FRLR) in Pittsburgh. The goal of his research is to enable fully immersive remote communication and interaction in the virtual world at a level that is indistinguishable from reality. One challenge is photo-realistic digitization and efficient rendering of digital humans. He develops key technology that combines fundamental computer vision, machine learning, and graphics techniques in a new neural capture and rendering paradigm. Before joining FRLR, Michael was a Visiting Assistant Professor at Stanford University and a Postdoctoral Researcher at the Max Planck Institute for Informatics. He received his PhD in 2014 from the University of Erlangen-Nuremberg for his work on real-time static and dynamic scene reconstruction.

\noindent 
\textbf{Vladislav Golyanik} leads the 4D and Quantum Vision research group at the Visual Computing and Artificial Intelligence Department of the Max Planck Institute for Informatics (MPII), Saarbrücken, Germany. The primary research interests of his team include 3D reconstruction and analysis of deformable scenes, matching problems on point sets and graphs, neural rendering, quantum computer vision and event-based vision. He received a doctoral degree in informatics from the University of Kaiserslautern in 2019, advised by Didier Stricker. Prior to joining MPII as a post-doctoral researcher, Vladislav was a visiting fellow at NVIDIA (San Jos\'e, USA), and Institute of Robotics and Industrial Informatics (Barcelona, Spain). He is the recipient of the WACV’16 best paper award and the 2020's yearly dissertation award of the German Association for Pattern Recognition (DAGM). 




==> draft.tex <==
\section{Neural Volumetric Rendering}

\subsection{Pre-NeRF Volume Rendering ML}
\BM{Should acknowledge prior view synthesis work from 2015-2020 such as Soft 3D, DeepStereo, Stereo Magnification, Neural Volumes, etc. Potentially also ML work focused on 3D reconstruction but that uses an alpha-compositing rendering model through a voxel grid, eg. some work by Shubham Tulsiani, Abhishek Kar, Philipp Henzler.}


\subsection{NeRF}
\subsection{Extensions to NeRF}
\subsubsection{Accelerations of 'Inference'}
\JB{I assume this is meant to cover things like \url{https://microsoft.github.io/FastNeRF/}, \url{https://phog.github.io/snerg/}, \url{https://github.com/creiser/kilonerf}, \url{https://alexyu.net/plenoctrees/}?}

\subsubsection{Accelerations of Training (meta networks)}
\JB{I don't think of meta networks as being synonymous with accelerating training (there are many other ways to accelerate training, and meta networks are often not used for speed). Thinking of them as "amortized inference" techniques makes sense to me, though I think we may want something that means "NeRFs wrapped inside other models".}

\subsubsection{Quality}
\JB{Maybe "Fidelity"?}

\subsubsection{Dynamics}
\JB{Is there a heading that captures the union of "Dynamic" and "Deformable" and "unknown cameras"? These all seem like basically the same problem to me (solving for the camera is a special case of deformation where the deformation field is a camera's projective, dynamic is a special case of deformable where things are on a 1D space, etc.)}

\subsubsection{Relighting/Path Tracing}
\JB{Maybe "Inverse Rendering"? NeRF is already tracing paths, and relighting is just one small function of an inverse rendering system (alongside material editing, view synthesis, various recognition things).}

\section{Engineering Techniques}

\CL{I think it would be great to also include at least a short discussion of frameworks and techniques that are great for efficiently implementing all types of aforementioned models---in particular since training them can be quite cumbersome if not done right. This could include JaxNeRF, EnzymeAD, \ldots}

\section{The Applications of Neural Rendering}
Each subsection discusses all applications : relighting, novel view synthesis....

\subsection{Novel View Synthesis (Static Scenes)}
\subsection{Novel View Synthesis (Dynamic Scenes)}
\subsection{Generalizable Scenes}
\subsection{Relighting}
\subsection{Human Specific}
\subsection{Generative Models}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Papers to Cover}

\begin{itemize}
    \item explicit~\cite{sitzmann2019deepvoxels,Lombardi:2019}
    \item implict / coordinate networks / MLPs~\cite{park2019deepsdf,mescheder2019occupancy}
    \item positional encoding~\cite{Mildenhall_2020_NeRF,tancik2020fourfeat}, SIREN~\cite{sitzmann2020siren}
    \item training strategies: progressive encoding~\cite{hertz2021sape}, multi-resolution~\cite{martel2021acorn} 
    \item generalization via conditioning by concatenation~\cite{mescheder2019occupancy,park2019deepsdf}, hypernetworks~\cite{sitzmann2019srns}, meta learning~\cite{sitzmann2019metasdf,tancik2020learned}, or modulation / feature-wise linear transforms~\cite{chanmonteiro2020piGAN,chen2020learning,mehta2021modulated}. 
\end{itemize}


\begin{itemize}
    \item proxy geometry with ray interpolation~\cite{gortler1996lumigraph,buehler2001unstructured}
    \item proxy geometry with on-surface feature aggregation / interpolation~\cite{riegler2020free,riegler2020stable}
    \item optimized neural surfaces with sphere tracing~\cite{Niemeyer2020CVPR,yariv2020multiview,kellnhofer2021neural} or volume rendering~\cite{oechsle2021unisurf}
\end{itemize}


\MZ{
\begin{itemize}
\item DeepVoxels~\cite{sitzmann2019deepvoxels}, Neural Volumes \cite{Lombardi_2019_NeuralVolumes}
\item MVP \cite{Lombardi_2021_MVP}
\item NeRF \cite{Mildenhall_2020_NeRF}
\item ... add more ...
\end{itemize}
}
\AT{
Deformable/Dynamic:
\begin{itemize}
    \item Non-Rigid NeRF \cite{tretschk2021nonrigid}
    \item Nerfies \cite{park2021nerfies}
    \item Dynamic View Synthesis from Dynamic Monocular Video \cite{Gao-freeviewvideo}
    \item Space-time Neural Irradiance Fields for Free-Viewpoint Video \cite{xian2021space}
    \item Neural scene flow fields for space-time view synthesis of dynamic scenes \cite{li2021neural}
    \item Neural Radiance Flow for 4D View Synthesis and Video Processing \cite{du2021nerflow}
    \item D-NeRF \cite{pumarola2020d}
\end{itemize}}

\AT{Portraits:
\begin{itemize}
    \item NeRFace \cite{Gafni_2021_CVPR}
    \item Learning Compositional Radiance Fields of Dynamic Human Heads \cite{wang2020learning}
    \item Pixel-aligned Volumetric Avatars \cite{raj2020pva}
    \item Portrait Neural Radiance Fields from a Single Image \cite{Gao-portraitnerf}
\end{itemize}}

\CL{
\begin{itemize}
    \item NeRF++: Analyzing and Improving Neural Radiance Fields~\cite{Zhang2020}
    \item NeRF in the Wild: Neural Radiance Fields for Unconstrained Photo Collections~\cite{Martin-Brualla2020}
    \item Neural 3D Video Synthesis~\cite{Li2021}
    \item Space-time Neural Irradiance Fields for Free-Viewpoint Video~\cite{Xian2020}
    \item Neural Scene Graphs for Dynamic Scenes~\cite{Ost2020}
\end{itemize}
Human bodies:
\begin{itemize}
    \item Animatable Neural Radiance Fields for Human Body Modeling~\cite{peng2021animatable},
    \item AD-NeRF: Audio Driven Neural Radiance Fields for Talking Head Synthesis~\cite{guo2021adnerf}
    \item Neural Body: Implicit Neural Representations With Structured Latent Codes for Novel View Synthesis of Dynamic Humans~\cite{Peng_2021_CVPR}
    \item A-NeRF: Surface-free Human 3D Pose Refinement via Neural Rendering~\cite{su2021anerf}
    \item PaMIR~\cite{Zheng2021}
    \item NARF: Neural Articulated Radiance Fields~\cite{Noguchi2021}
\end{itemize}
Faces:
\begin{itemize}
    \item Dynamic Neural Radiance Fields for Monocular 4D Facial Avatar Reconstruction~\cite{Gafni2020}
    \item Learning Compositional Radiance Fields of Dynamic Human Heads~\cite{Wang2020}
\end{itemize}
Relaxed assumptions:
\begin{itemize}
    \item INeRF: Inverting Neural Radiance Fields for Pose Estimation~\cite{Yen-Chen2020}
    \item NeRF--: Neural Radiance Fields Without Known Camera Parameters~\cite{wang2021nerfmm}
    \item ShaRF: Shape-conditioned Radiance Fields from a Single View~\cite{Rematas2021}
    \item pixelNeRF: Neural Radiance Fields from One or Few Images~\cite{Yu2020}
    \item NeRF-VAE: A Geometry Aware 3D Scene Generative Model~\cite{Kosiorek2021}
    \item CAMPARI: Camera-Aware Decomposed Generative Neural Radiance Fields~\cite{Niemeyer2021}
\end{itemize}
Lighting:
\begin{itemize}
    \item NeRV: Neural Reflectance and Visibility Fields for Relighting and View Synthesis~\cite{Srinivasan2020}
    \item NeRD: Neural Reflectance Decomposition from Image Collections~\cite{Boss2020}
\end{itemize}
Representations:
\begin{itemize}
    \item Learned Initializations for Optimizing Coordinate-Based Neural Representations~\cite{Tancik2020}
    \item AutoInt: Automatic Integration for Fast Neural Volume Rendering~\cite{Lindell2020}
    \item FastNeRF: High-Fidelity Neural Rendering at 200FPS~\cite{Garbin2021}
    \item NeX: Real-time View Synthesis with Neural Basis Expansion~\cite{Wizadwongsa2021}
    \item Pulsar: Efficient Sphere-based Neural Rendering~\cite{Lassner_pulsar}
    \item Neural Sparse Voxel Fields~\cite{Liu2020}
    \item DONeRF: Towards Real-Time Rendering of Compact Neural Radiance Fields using Depth Oracle Networks~\cite{Neff2021}
    \item KiloNeRF: Speeding up Neural Radiance Fields with Thousands of Tiny MLPs~\cite{Reiser2021}
    \item DeRF: Decomposed Radiance Fields~\cite{Rebain2020}
    \item PlenOctrees for Real-time Rendering of Neural Radiance Fields~\cite{Yu2021}
    \item Unconstrained Scene Generation with Locally Conditioned Radiance Fields~\cite{DeVries2021}
    \item GRAF: Generative radiance fields for 3D-aware image synthesis~\cite{Schwarz2020}
    \item pi-GAN: Periodic Implicit Generative Adversarial Networks for 3D-Aware Image Synthesis~\cite{Chan2020}
    \item GIRAFFE: Representing Scenes as Compositional Generative Neural Features Fields~\cite{Niemeyer2020}
    \item GRF: Learning a General Radiance Field for 3D Representation and Rendering~\cite{Trevithick2020}
    \item Object-Centric Neural Scene Rendering~\cite{Guo2020}
    \item IBRNet: Learning Multi-View Image-Based Rendering~\cite{Wang}
\end{itemize}
Others:
\begin{itemize}
    \item Enzyme AD~\cite{NEURIPS2020_9332c513}
    \item In-Place Scene Labelling and Understanding with Implicit Scene Representation~\cite{Zhi2021}
    \item iMAP: Implicit Mapping and Positioning in Real-Time~\cite{Sucar2021}
\end{itemize}}


\begin{itemize}
    \item code-nerf
    \item object-nerf
    \item nerf-tex
\end{itemize}

%
% \section{Neural Rendering using 2D Representations}

% \MZ{Is it really GANs? More like image-to-image translation in general? Or screen-space method?}
% \MZ{Not sure, but I still feel we should get rid of these and have a strong 3D focus}

% Each subsection discusses all applications : relighting, novel view synthesis....

% \subsection{Unconditional GANs}
% \MZ{Generative models?}
% pi-GAN, StyleRig,....

% \subsection{Conditional GANs}
% MPI Tuebingen, Samsung papers...

% \section{Neural Rendering using 3D Representations}
% %
% Each subsection discusses all applications : relighting, novel view synthesis....
% \subsection{Surface Representations}
% Lumigraph Rendering,...

% \subsection{Volumetric Representations}
% Most of the paper.



==> tables/table_compositional.tex <==
    
\begin{table}
    \centering
    %\small
    %\scalebox{0.9}{
    \begin{adjustbox}{max width=\linewidth}
    
    \centering
    \begin{tabular}{lccccc}
        \toprule
        Method &
        \rot{Required Data} &           % monocular image, video (dynamic content), multiview images (static content) + illumination
        \rot{3D Representation} &       % surface (SDF, mesh etc.), or volumetric (density)
        \rot{Controllable Parameters} & % viewpoint, illumination, time, deformation, material
        \rot{Generative Model} &        % generative
        \rot{Code} \\                   % link to code

        
        % compositionality / editing 
        
        
        \midrule
        Nguyen-Phuoc \etal~\cite{nguyen2019hologan} 
        & \opC{MVI}+\opD{UIC} & \opA{V}  & \opA{P},\opB{S},\opC{T}  & \cmark{}  & \code{https://github.com/thunguyenphuoc/HoloGAN}  
        \\
        \cmidrule(lr){1-6}
        Liu~\etal~\cite{liu2021editing}
        & \opC{MVI} & \opA{V}  & \opB{S},\opE{C}   & \xmark{}  & \code{https://github.com/stevliu/editnerf}            
        \\
        
        \cmidrule(lr){1-6}
        Jang and Agapito~\cite{Jang_2021_ICCV}
        & \opD{UIC} & \opA{V}  & \opA{P},\opB{S},\opC{T}  & \xmark{}  & \code{https://github.com/wayne1123/code-nerf}        
        \\
        \midrule
        Ost~\etal~\cite{Ost2021}
        & \opA{VID} & \opB{V-O}  & \opA{P},\opB{S},\opC{T},\opD{O}  & \cmark{}  & \code{https://github.com/princeton-computational-imaging/neural-scene-graphs}  
        \\
        \cmidrule(lr){1-6}
        Zhang~\etal~\cite{zhang2021stnerf}
        & \opB{MV-VID} & \opB{V-O}  & \opB{S},\opE{C}  & \cmark{}  & \code{https://github.com/DarlingHang/ST-NeRF}          
        \\
        \cmidrule(lr){1-6}
        Niemeyer and Geiger~\cite{niemeyer2020giraffe}
        & \opD{UIC} & \opC{NFF}  & \opA{P},\opB{S},\opC{T} & \cmark{}  & \code{https://github.com/autonomousvision/giraffe} 
        \\
        
   \end{tabular}
   %}
   \end{adjustbox}
    
    \caption{Selected methods for editing and scene compositionality presented in \Cref{sec:compedit}. 
    % 
    \tableopt{opA}{VID}:~Monocular videos, 
    \tableopt{opB}{MV-VID}:~Synchronised multi-view videos, 
    \tableopt{opC}{MVI}:~Multi-view image collections, 
    \tableopt{opD}{UIC}:~Unstructured 2D image collections.
    \tableopt{opA}{V}:~Neural volumetric, 
    \tableopt{opB}{V-O}:~Per-object+background neural volumetric, 
    \tableopt{opC}{NFF}:~Neural feature fields.
    \tableopt{opA}{P}:~Camera pose,
    \tableopt{opB}{S}:~Shape, 
    \tableopt{opC}{T}:~Texture/appearance, 
    \tableopt{opD}{O}:~Opacity,
    \tableopt{opE}{C}:~Color.
    % See \Cref{sec:compedit} for explanation of attributes in the table and their possible values. 
    % 
    }
    \label{tbl:overview_compedit}
\end{table}

==> tables/table_novel_view.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
    \centering
    %\small
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccccc}
        \toprule
        Method &
        \rot{Required Data} &
        \rot{Requires Pre-trained NeRF} &
        \rot{3D Representation} & 
        \rot{Persistent 3D} & 
        \rot{Network Inputs} &          % coordinates vs. positional encoded coordinates vs. learned embedding
        %\rot{Training Time} &           % 
        %\rot{Inference Speed} &         % real-time, non-real-time
        \rot{Code} \\                   % link to code
        
        % static novel view-point synthesis
        \midrule
        Mildenhall~\etal~\cite{Mildenhall_2020_NeRF}
        & \opA{I}+\opB{P} & \xmark{} & \opB{V} & \opA{F} 
        & \opD{PE}(\opA{P})+\opD{PE}(\opF{V})  &  \code{https://github.com/bmild/nerf} 
        \\
        
        \cmidrule(lr){1-7}
        Sitzmann~\etal~\cite{sitzmann2019srns}
        & \opA{I}+\opB{P} & \xmark{} & \opC{S} & \opF{P}      
        & \opA{P} &  \code{https://github.com/vsitzmann/scene-representation-networks} 
        \\
        
        \cmidrule(lr){1-7}
        Niemeyer~\etal~\cite{Niemeyer2020CVPR}
        & \opA{I}+\opB{P}+\opD{M} & \xmark{} & \opD{O} & \opA{F}      
        & \opA{P} & \code{https://github.com/autonomousvision/differentiable_volumetric_rendering} 
        \\
        
        %\cmidrule(lr){1-7}
        %Park~\etal~\cite{park2019deepsdf}
        %& S & \xmark{} & S & F     
        %& P &  \code{https://github.com/facebookresearch/DeepSDF} 
        %\\
        
        %\cmidrule(lr){1-7}
        %Mescheder~\etal~\cite{mescheder2019occupancy}
        %& S & \xmark{} & O & F     
        %& P &  \code{https://github.com/autonomousvision/occupancy_networks}
        %\\
        
        \cmidrule(lr){1-7}
        Chen~\etal~\cite{chen2019learning}
        & \opC{S} & \xmark{} & \opD{O} & \opA{F}      
        & \opA{P} &  \code{https://github.com/czq142857/implicit-decoder} 
        \\
        
        \cmidrule(lr){1-7} 
        Gu~\etal~\cite{liu2020neural} 
        & \opA{I}+\opB{P} & \xmark{} & \opA{G}+\opB{V} & \opA{F} 
        & \opD{PE}(\opA{P})+\opD{PE}(\opF{V}) &  \code{https://github.com/facebookresearch/NSVF} 
        \\
        
        \cmidrule(lr){1-7}
        Lindell~\etal~\cite{lindell2020autoint}
        & \opA{I}+\opB{P} & \xmark{} & \opB{V} & \opF{P}      
        & \opD{PE}(\opA{P})+\opD{PE}(\opF{V}) & \code{https://github.com/computational-imaging/automatic-integration}   
        \\
        
        \cmidrule(lr){1-7}
        Reiser~\etal~\cite{Reiser2021}
        & \opA{I}+\opB{P} & \cmark{} & \opA{G}+\opB{V} & \opA{F}     
        & \opD{PE}(\opA{P})+\opD{PE}(\opF{V}) & \code{https://github.com/creiser/kilonerf} 
        \\
        
        \cmidrule(lr){1-7}
        Garbin~\etal~\cite{garbin2021fastnerf}
        & \opA{I}+\opB{P} & \cmark{} & \opA{G} & \opA{F}      
        & \opA{P}+\opF{V} & \xmark{}       
        \\
        
        \cmidrule(lr){1-7}
        Hedman~\etal~\cite{hedman2021snerg}
        & \opA{I}+\opB{P} & \cmark{} & \opA{G} & \opA{F}      
        & \opA{P}+\opD{PE}(\opF{V}) & \code{https://github.com/google-research/google-research/tree/master/snerg}         
        \\
        
        \cmidrule(lr){1-7}
        Yu~\etal~\cite{yu2021plenoctrees}
        & \opA{I}+\opB{P} & \cmark{} & \opA{G} & \opA{F}      
        & \opA{P}+\opF{V} & \code{https://github.com/sxyu/plenoctree}
        \\
        
        \cmidrule(lr){1-7}
        Neff~\etal~\cite{Neff2021}
        & \opA{I}+\opB{P}+\opE{D} & \xmark{} & \opB{V} & \opA{F}      
        & \opD{PE}(\opA{P})+\opD{PE}(\opF{V}) & \code{https://github.com/facebookresearch/DONERF}     
        \\
        
        \cmidrule(lr){1-7}
        Sitzmann~\etal~\cite{sitzmann2021lfns}
        & \opA{I}+\opB{P} & \xmark{} & \xmark{} & \opC{N}      
        & \opC{L} & \code{https://github.com/vsitzmann/light-field-networks}         
        \\
            \end{tabular}
    \end{adjustbox}
    \caption{Selected methods for static scene view synthesis presented in \Cref{sec:static_nvp}. Although some of these representations are used for applications beyond static scene view synthesis, in this table we only classify such methods based on the use of their underlying 3D scene representation for static scene view synthesis. %See \Cref{sec:applications} for explanation of attributes in the table and their possible values. 
        %%
        \tableopt{opA}{I}:~Images,
        \tableopt{opB}{P}:~Camera poses (exact or approximate),
        \tableopt{opC}{S}:~3D shape,
        \tableopt{opD}{M}:~Object masks,
        \tableopt{opE}{D}:~Depth.
        \tableopt{opA}{G}:~Grid,
        \tableopt{opB}{V}:~Neural volumetric,
        \tableopt{opC}{S}:~Neural SDF,
        \tableopt{opD}{O}:~Neural occupancy.
        \tableopt{opA}{F}:~Fully,
        \tableopt{opF}{P}:~Partial,
        \tableopt{opC}{N}:~Not guaranteed.
        \tableopt{opA}{P}:~3D position,
        \tableopt{opF}{V}:~2D viewing direction,
        \tableopt{opC}{L}:~Light field ray coordinates.
        \tableopt{opD}{PE}():~Positinal encoding of argument.
        %%
    % \AT{Are there many papers which are covered both in generalization and novel view synthesis? If so, we could merge the tables. }
    } 
    %\ET{TODO: fill out Training Time and Inference Speed columns} 
    %\VG{symbols \opB{P} and \opB{V} are repeated} 
    %\AT{true, we should assign different colors if they represent different things}
    \label{tbl:overview_novel_view}
\end{table}


==> tables/table_relighting.tex <==

\begin{table}
    \centering
    %\small
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccccc}
        \toprule
        Method &
        \rot{Required Data} &           
        \rot{3D Representation} &       
        \rot{Controllable Parameters} & 
        \rot{Models Light Visibility} &  
        \rot{Models Indirect Illumination} &  
        \rot{Code} \\                   % link to code
        
        % relighting and material editing
        \midrule
        Bi~\etal~\cite{bi2020nrf}
        & \opA{I}+\opB{L} & \opA{V} & \opA{L}+\opB{M} & \cmark{} & \xmark{} & \xmark{}
        \\
        \cmidrule(lr){1-7}
        Zhang~\etal~\cite{zhang2021physg}
        & \opA{I}+\opC{M} & \opB{S} & \opA{L}+\opB{M} & \xmark{} & \xmark{} & \code{https://github.com/Kai-46/PhySG}       
        \\
        
        \cmidrule(lr){1-7}
        Boss~\etal~\cite{boss2020nerd}
        & \opA{I}+\opC{M} & \opA{V} & \opA{L}+\opB{M} & \xmark{} & \xmark{} &    \code{https://github.com/cgtuebingen/NeRD-Neural-Reflectance-Decomposition}   
        \\
        
        \cmidrule(lr){1-7}
        Srinivasan~\etal~\cite{srinivasan2021nerv}
        & \opA{I}+\opB{L} & \opA{V} & \opA{L}+\opB{M} & \cmark{} & \cmark{} & \xmark{}           
        \\
        
        \cmidrule(lr){1-7}
        Zhang~\etal~\cite{zhang2021nerfactor}
        & \opA{I} & \opA{V} & \opA{L}+\opB{M} & \cmark{} & \xmark{} & \code{https://github.com/google/nerfactor} 
        \\
        
        \cmidrule(lr){1-7}
        Xiang~\etal~\cite{xiang2021neutex}
        & \opA{I}+\opC{M} & \opA{V} & \opC{T} & N/A & N/A & \xmark{}         
        \\



        %\midrule
        %\noalign{\vskip 0.01cm}  
        %\cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-11}
        %& \multicolumn{4}{c}{Inputs and Outputs} & \multicolumn{2}{c}{Control} & \multicolumn{4}{c}{Misc} & \\
        %\noalign{\vskip 0.01cm}
        %\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Selected methods for relighting presented in \Cref{sec:relight}.
    %%
            \tableopt{opA}{I}:~Images,
            \tableopt{opB}{L}:~Lighting parameters for input images,
            \tableopt{opC}{M}:~Object masks.
            \tableopt{opA}{V}:~Neural volumetric,
            \tableopt{opB}{S}:~Neural SDF.
            \tableopt{opA}{L}:~Lighting,
            \tableopt{opB}{M}:~Materials,
            \tableopt{opC}{T}:~Texture map.
            %%
    }
    \label{tbl:overview_relight}
\end{table}


==> videos_tali_backup.tex <==
\section{Video Synthesis and Editing}\label{sec:video}
\Authors{Tali, Gordon + support team}

\jon{I'd like to see some commentary on the difficulty in explicitly controlling video models}


\noindent
\Suggestions{
Try to have a consistent thread shared among all subfields, e.g.
\begin{itemize}
    \item Definition of the task and significance.
    \item In the context of the general challenges (such as data, dimensionality) and specific challenges for this domain, provide more references and specific solutions if needed.
    \item Highlight data source and public available codebases including community repos.
    \item Discussion paragraph: Open challenges
    \item Comparison to state-of-the-art in the field as a whole (not only diffusion methods)
\end{itemize}
}

\textcolor{red}{Figures to include}:
\begin{itemize}
    \item schematic of temporal attention, perhaps from \cite{ho2022video} (done)
    \item examples of video editing (maybe one example illustrating the conditioning approach and one for feature warping? (TODO)
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

\par\rule{\columnwidth}{0.5pt} 

Text-to-video (T2V) diffusion models extend text-to-image (T2I) models by using a diffusion model to generate a (short) video given only a text prompt, a single image (e.g., with additional conditioning data such as optical flow), or an input video. The last setting, video-to-video translation, is closely related to conventional video editing, and often involves alterations of the input video in the latent space of a pre-trained T2V model.

The first challenge for all T2V models is to model the temporally consistent structure of video without compromising on the quality of the underlying T2I models. Usually, this is achieved by extending T2I U-Net architectures to 3D by introducing separable temporal layers, usually using temporal convolutions and temporal attention mechanisms (see Fig.~\ref{fig:video:spatiotemporalunet}). 

The second challenge for T2V models is to train them. Here, we differentiate between two approaches: (i) methods that train or fine tune a T2V model using a large dataset of videos scraped from the web and (ii) methods that build directly on pre-trained text-to-image models in a zero-shot/one-shot setting, i.e., they do not use any video data to train or refine the model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Video Generation}
\tali{Despite the tremendous progress in \emph{image} diffusion models, and the remarkable breakthroughs in text-to-image generation, expanding this progress to the domain of  \emph{video}  is still in nascent stages, due to two main challenges. \\ \\ First, learning from videos require order of magnitude more data than images, due to the complexity and diversity of our dynamic world. While online videos are abundant, curating high-quality video datasets remain a difficult task that typically involves significant engineering efforts and requires dedicated automatic curation tools. \\ \\
Another substantial challenge arises from the high dimensionality of raw video data, e.g.,  a 2 minutes video taken at 30fps consists of 3600× more pixels than a single frame. This makes the extension of 2D architectures to the temporal domain extremely challenging and computationally expensive. We next discuss how these challenges have been tackled in the context of diffusion models.  }
%Text-to-video models -- extension of image models to video through separable temporal layers (typically temporal convs and temporal attention), trained/finetuned on a dataset of videos: 


% also check recent discussion of this work in https://arxiv.org/pdf/2307.06940.pdf
% two open-sourcing text2video generation models ModelScope [damo vilab 2023] and LVDM [He et al. 2022].

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/video_spatio_temporal_unet.jpg}
    \caption{(A) Common attention U-Net used for the denoising step in image and video diffusion models comprising residual convolution blocks and attention blocks as well as concatenated time step and text prompt--embeddings. Figure adapted from \cite{Kochanowicz}. (B) Temporal structure in video diffusion and editing is commonly modeled by adding 1D temporal convolutions in the residual blocks (left) as well as 1D temporal attention blocks after each of the 2D spatial attention blocks (right). Figure adapted from \cite{esser2023structure}.}
    \label{fig:video:spatiotemporalunet}
\end{figure}

%References to discuss:
%\begin{itemize}
    %\item Video Diffusion Models (VDM) \cite{ho2022video} introduced the first large-scale T2V diffusion model. They extended the common Unet-based T2I architecture by adding temporal (attention) layers. Trained jointly on videos and individual frames.  Classifier-free guidance to improve sample quality for text conditioned generation; a 3D U-Net, factorized over space and time \cite{cciccek20163d}
    %\item Make-a-Video \cite{singer2022make} finetune a pre-trained T2I diffusion only on videos. They added temporal layers, trained the entire network. They train their network on unlabeled videos (i.e., without text captions). This allows them to train on large-scale available video dataset.
    %\item Similarly to T2I, high-resolution T2V is achieved by training in a low-resolution latent space (LDM approach) \cite{blattmann2023align,wang2023modelscope} or by training cascaded models \cite{ho2022imagen}. 
    %\item ~\cite{esser2023structure} trains a video diffusion model that is particularly well suited for video editing; Spatio-temporal Latent Diffusion; add a 1D temporal convolution after each 2D spatial convolution in its residual blocks, and we add a 1D temporal attention block after each of its 2D spatial attention blocks; Gen-1 presents a large scale video generation model that uses depth as a structural cue. The model is trained on a large, mixed dataset of images and videos.
    %\item  AnimateDiff \cite{guo2023animatediff} train temporal attention layers, that can be plugged in on off-the-shelf SD models (e.g., finetuned on videos from specific styles).
    %\item VideoFusion \cite{luo2023videofusion} decouples per-frame noise into base noise and residual noise, which benefits from a well-pretrained DALL-E 2 and provides better control over content and motion;  we present a decomposed DPM for video generation (VideoFusion). It decomposes the standard diffusion process as adding a base noise and a residual noise, where the base noise is shared by consecutive frames
%\end{itemize}

\paragraph*{Training and Refining Diffusion Models with Large-scale Video Data.}
\tali{I think I prefer Unconditional and Text-Conditioned Video Diffusion Models}


Video Diffusion Models (VDMs)~\cite{ho2022video} introduced the first T2V diffusion model. Imagen Video~\cite{ho2022imagen} introduced a cascaded model that initially models video distribution at low resolution and then applies spatio-temporal interpolation to increase the resolution and time duration. Both VDM and Imagen Video are developed by Google. These T2V models as well as Gen-1~\cite{esser2023structure} by Runway ML are trained jointly on a large corpus of videos and individual frames and rely on classifier-free guidance for generating high-fidelity samples which respect a given text prompt. Make-A-Video~\cite{singer2022make} and Make-a-Video-4D~\cite{Singer2023TextTo4DDS} (see more details in Sec.~\ref{sec:4D_generation}) by Meta AI, Align-your-Latents~\cite{blattmann2023align} by Nvidia, MagicVideo~\cite{zhou2022magicvideo} by ByteDance, and ModelScope~\cite{wang2023modelscope} by Alibaba all fine-tune pre-trained T2I diffusion models on large amounts of unlabeled (i.e., without text captions) or sparsely labeled video data.  AnimateDiff~\cite{guo2023animatediff} follows a similar strategy and discusses personalization strategies of the Base T2I model in depth. Most of these approaches extend existing T2I models using a 3D U-Net architecture~\cite{cciccek20163d} that is factorized over space and time by adding temporal convolution and attention layers. A representative illustration of this architecture is shown in Fig.~\ref{fig:video:spatiotemporalunet}.

Align-your-Latents and MagicVideo adopt a latent diffusion strategy for high-resolution and computationally efficient video generation. PVDM~\cite{yu2023video}, Latent Video Diffusion Models~\cite{he2022latent}, and VideoGen \cite{li2023videogen} also propose different variants of latent video diffusion strategies.

Other approaches to video generation include MCVD~\cite{voleti2022MCVD}, which generates videos autoregressively by conditioning new frames on previously generated frames, and VideoFusion~\cite{luo2023videofusion}, which decomposes the noisy latents of the video into the sum of a (static) base noise and a (dynamic) residual noise.

\paragraph*{Zero- and One-shot Tuning of T2I Models.}
%
%On the other side of the spectrum, one-shot/zero-shot adaptation of T2I to video generation:
%\begin{itemize}
    %\item Tune-A-Video \cite{wu2022tune} inflate SD and fine-tune it on a single video. Used for video editing; \tali{was debating if Tune-A-Video should go here or in the video editing section.} \gordon{we can use it in both subsections}
    %\item \cite{khachatryan2023text2video} generate clip from SD without any video finetuning: they extend the self-attention module to operate jointly on several frames (aka extended attention) and perform simple manipulations on the noise latents to encourage consistency.
    %\item SceneScape \cite{Fridman2023SceneScapeTC}; generate a 3D-consistent walkthroughs videos that comply with a given text. 
    %\item Make-a-Video-4D \cite{Singer2023TextTo4DDS} optimize a 4D representation (cite) using score-distillation loss (cite SDS): motion from a T2V model, 2D prior from a T2I model. Ensures consistent geometry.
    %\item SinFusion \cite{NikankinHI23} -- trains a diffusion model on a single video from scratch. No external priors learned from a dataset.    
%\end{itemize}

Although large-scale video datasets are readily available on the web, training a T2V model is computationally expensive. Several recent approaches propose to fine-tune a T2I model in a zero-shot setting, i.e., given no additional data, or a one-shot setting, i.e., given a single video, and then generate videos or variations of the input video, changing style, structure, layout, or other aspects.

Text2Video-Zero~\cite{khachatryan2023text2video} generates video clips using Stable Diffusion without any video fine tuning in a zero-shot setting. They extend the self-attention module to operate jointly on several frames and perform simple manipulations on the noise latents to encourage consistency.

One-shot approaches require a single video as input. Tune-A-Video~\cite{wu2022tune}, for example, inflates Stable Diffusion into the temporal domain and fine-tunes it on a single video. This method is primarily used for video editing application, as discussed in the following subsection. Fate/Zero~\cite{qi2023fatezero} inverts an input video into latents of a text-to-image diffusion model and re-generates it with temporally consistent editing options. SinFusion~\cite{NikankinHI23} trains a diffusion model on a single video from scratch and is shown to enable diverse variations of this video to be generated, in addition to video extrapolation, retargeting, and temporal upsampling. 

Inspired by the perpetual view generation problem introduced by Infinite Nature~\cite{infinite_nature_2020,li2022_infinite_nature_zero}, several methods recently proposed diffusion models for this task. For example, given only a text prompt, SceneScape~\cite{Fridman2023SceneScapeTC} generates 3D-consistent scenes rendered from a specified camera trajectory flying out of the scene. DiffDreamer~\cite{cai2023diffdreamer} takes a single input image and generates renderings of a specified camera trajectory flying into the scene. Although these tasks seem similar, flying into a scene is more challenging because this problem not only requires 3D-multi-view consistent out-painting but also super-resolution, as novel details of a previously seen structure become visible in later frames.

% \begin{itemize}
%     \item fine-tuning T2I models for video generation by
%     \begin{itemize}
%     \item updating all or most model parameters \cite{ho2022video,esser2023structure,singer2022make,wu2022tune,zhou2022magicvideo}
%     \item training-free by latent warping with affine matrix \cite{khachatryan2023text2video}
%     \item train separate motion layers in T2I model \cite{blattmann2023align}
%     \item ...
%     \end{itemize}
%     \item \cite{ho2022imagen,singer2022make,zhou2022magicvideo,hong2022cogvideo}
%     \item also \cite{wu2021godiva,wu2022nuwa}
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Video Editing based on Video-to-Video Diffusion \tali{maybe replace to: Controlled Video Generation and Editing?}}

%Various methods for video editing/controlled video generation (e.g., conditioning on spatial input such as depth maps). All extend/adapt/initialize from a T2I model: 
%\begin{itemize}
    %\item Runway GEN-1 \cite{esser2023structure} train a video diffusion model that is conditioned on structure (depth) and appearance representations (CLIP image embedding) for text-driven video-to-video translation. 
    %\item VideoComposer~\cite{wang2023videocomposer} extends Composer \cite{huang2023composer} to videos by  training a conditional video model that is conditioned on a variety of per-frame spatial controls (e.g., sketches, depth, motion scribbles, CLIP image embedding); trained on large-scale video dataset.  
    %\item Similar to VideoComposer; Control-A-Video \cite{chen2023controlavideo} extend ControlNet \cite{zhang2023adding}, train on videos, add temporal attention.
    %\item \cite{He2023AnimateAStorySW} retrieve depth maps from a database given the target prompt, and use them for conditional generation.
    %\item DreamMix \cite{molad2023dreamix} utilize ImagenVideo \cite{ho2022imagen} for video editing. 
    %\item MagicEdit \cite{liew2023magicedit} train an image-based ControlNet over a T2I model. Then train temporal attention over a fixed T2I. Combine the ControlNet with the trained temporal attentnio layers -- allowing various editing capabilities (image to video, depth to video, outpainting etc.)
    %\item Use fixed T2I model editing a given video: all extended attention-based methods \cite{}, TokenFlow~\cite{tokenflow2023}.
    %\item Other: VideoP2P \cite{liu2023videop2p}, Fate/Zero \cite{qi2023fatezero}
%\end{itemize}


%Pre-trained video diffusion models, such as those discussed in the previous subsection, can be readily used for video editing. For example, Runway's Gen-1 model~\cite{esser2023structure} is specifically designed to enable high-quality text-driven video-to-video translation. 
\tali{Like with images, an important aspect in leveraging generative video models in real-world content creation tasks, is the ability to provide users with various controls over the generated content. }
Various methods for video editing or controlled video generation have been proposed. We discuss several approaches, with their relative benefits and disadvantages, in the following.

\paragraph*{Conditioning.}

ControlNet~\cite{zhang2023adding} is a popular approach to condition the image generation process, for example using guidance from edges, poses, or semantic labels. This idea has recently been extended to video generation and editing scenarios. For example, Runway's Gen-1 model~\cite{esser2023structure} is specifically designed to enable high-quality text-driven video-to-video translation by conditioning the generation process on depth maps and text. VideoComposer~\cite{wang2023videocomposer} is a video generation model that is conditioned on a variety of per-frame spatial controls (e.g., motion vectors extracted from videos, sketches, depth, motion scribbles, CLIP image embedding). Control-A-Video~\cite{chen2023controlavideo} introduced Video-ControlNet as an extension of ControlNet to the temporal domain. Text2Video-zero~\cite{khachatryan2023text2video}
extends text-to-image generation using conditioning on video motion dynamics as well as using edge, body pose, or depth guidance. Animate-a-Story~\cite{He2023AnimateAStorySW} retrieves depth maps from a database given the target prompt, and uses them for conditional video generation. MagicEdit~\cite{liew2023magicedit} also uses a ControlNet to condition the output of a text-to-image generation model extended with temporal attention layers to enable various video editing applications, including stylization, local editing, and video outpainting, and image-to-video generation. DreamMix~\cite{molad2023dreamix} utilizes ImagenVideo for text-guided video generation and editing conditioned on low-resolution spatio-temporal information from a driving video, for example to translate a single or multiple input images to a video.

\textcolor{red}{Discuss benefits and limitations of conditioning.}

\paragraph*{Video Editing via Fine-tuning.}

Tune-A-Video~\cite{wu2022tune} and VideoP2P~\cite{liu2023videop2p} propose to fine-tune a pre-trained text-to-image diffusion model for a specific target video. While enabling high-quality video edits, this is a computationally expensive approach, which requires fine tuning for each target video.

\paragraph*{Feature Editing and Warping.}

It has been shown that different features in diffusion models correspond to appearance (e.g., the input to the self-attention layers) or structure (e.g., the output of the self-attention layers), respectively~\textcolor{red}{CITE, prompt-to-prompt?}. This insight can be exploited to edit the style or appearance of a single frame, or a few keyframes, of a video and propagate these edits, in a temporally consistent manner, to other frames while preserving the structure and motion of the input. Importantly, image edits can be performed with any pre-trained text-to-image diffusion model and do not require training a dedicated text-to-video model or fine-tuning one. 

Along these lines, Pix2Video~\cite{ceylan2023pix2video} applies (text-conditioned) image editing on the first frame of a video and injects features obtained from the previously edited frames into the self-attention layer of the current frame in an autoregressive manner. TokenFlow~\cite{tokenflow2023} proposes to jointly edit a few keyframes of the input video and warp the output tokens from the self-attention modules to other frames based on the correspondences provided by the original video features.

Fate/Zero~\cite{qi2023fatezero} inverts an input video into latents of a text-to-image diffusion model augmented with spatial-temporal self-attention and cross-attention maps. These latents are diffused back into clean frames conditioned on target prompt, but the inverted attention maps are blended with the edited ones to maintain the structure and temporal dynamics of the input video.  


\textcolor{red}{Discuss benefits and limitations of feature warping.}

\paragraph*{Video-to-Layered-Image Decomposition.} Another related idea is to decompose an input video clip into one or a few canonical images with corresponding per-frame deformation fields. This approach allows (text-conditioned) image editing approaches (see Sec.~\textcolor{red}{XXX}) to be directly applied to the canonical image(s). Examples of this approach include Text2LIVE~\cite{bar2022text2live}, which achieves a very high quality by decomposing the input clip into layered neural atlases \cite{kasten2021layered}, shape-aware extensions of Text2LIVE~\cite{lee2023shape}, and CoDeF~\cite{ouyang2023codef}. A benefit of this approach is that temporal consistency is guaranteed by design. Limitations of these methods include the long processing times to decompose the input video as well as an inherent assumption these that the input clip can be decomposed into canonical images, which is not always the case.

\gordon{Should we potentially add some discussion / re-structure this part to emphasize which methods build only on a pretrained T2I model, which fine-tune on a single video, and which use a pre-trained T2V model?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Benchmarks, Datasets, and Metrics}

\paragraph*{Metrics.}

\begin{itemize}
    \item FVD \cite{unterthiner2018towards}
    \item KVD
    \item FID \cite{heusel2017gans}
    \item IS \cite{salimans2016improved}
    \item CLIP cosine similarity of consecutive frames for frame consistency
    \item average CLIP cosine similarity
between text and image embeddings over all frames for prompt consistency
    \item CLIP R-precision for text-to-3D generation \cite{poole2022dreamfusion}
\end{itemize}

- C3D network \cite{tran2015learning} for calculating FID and IS 
- FVD using the I3D network \cite{carreira2017quo}

\paragraph*{Benchmarks.}

List some public video datasets in addition to scraping. 

%LAION [50]. We utilize the LAION-5B dataset as image-text pairs, specifically the LAION2B-en subset, as the model focuses on English input. The LAION dataset encompasses objects, people, scenes, and other real-world elements.

%WebVid [2]. The WebVid dataset comprises almost 10 million video-text pairs, with a majority of the videos having a resolution of 336 × 596. Each video clip has a duration of approximately 30 seconds. During the model training, we selected the middle square portion and randomly picked 16 frames with 3 frames per second as training data.

%MSR-VTT [63]. The MSR-VTT dataset is used to validate our model performance and is not utilized for training. This dataset includes 10k video clips, each of which is annotated with 20 sentences. To obtain FID-vid and FVD metric results, 2,048 video clips were randomly selected from the test set, and one sentence was randomly chosen from each clip to generate videos. When evaluating on CLIPSIM metric, we followed previous works [51, 62] and use nearly 60k sentences from the whole test split as prompts to generate videos.

\begin{itemize}
    \item unconditional video generation
    \item video prediction (BAIR Robot Pushing and Kinetics-600)
    \item text-conditioned video generation
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Open Challenges}

\begin{itemize}
    \item metrics for temporal consistency?
\end{itemize}


